GIRAFFE: Design Choices for Extending the Context Length of Visual Language Models

Visual Language Models (VLMs) demonstrate impressive capabilities in processing multimodal inputs, yet applications such as visual agents, which require handling multiple images and high-resolution videos, demand enhanced long-range modeling. Moreover, existing open-source VLMs lack systematic exploration into extending their context length, and commercial models often provide limited details. To tackle this, we aim to establish an effective solution that enhances long context performance of VLMs while preserving their capacities in short context scenarios. Towards this goal, we make the best design choice through extensive experiment settings from data curation to context window extending and utilizing: (1) we analyze data sources and length distributions to construct ETVLM - a data recipe to balance the performance across scenarios; (2) we examine existing position extending methods, identify their limitations and propose M-RoPE++ as an enhanced approach; we also choose to solely instruction-tune the backbone with mixed-source data; (3) we discuss how to better utilize extended context windows and propose hybrid-resolution training. Built on the Qwen-VL series model, we propose Giraffe, which is effectively extended to 128K lengths. Evaluated on extensive long context VLM benchmarks such as VideoMME and Viusal Haystacks, our Giraffe achieves state-of-the-art performance among similarly sized open-source long VLMs and is competitive with commercial model GPT-4V. We will open-source the code, data, and models.

==> 04analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\mukai{add intro}
% % \subsection{what plays the key part for extending vlm length}
% % context length variance via context length for LVLM
\subsection{Tasks construction}

We divided the tasks into three main categories: single image test results, multi-image test results, and video test reuslts. For single image tasks, we chose MME~\citep{fu2023mme} and MMBench~\citep{liu2024mmbenchmultimodalmodelallaround}, which are widely used benchmarks that reflect the diverse capacities of VLMs.
For multi-image testing, we follow LLaVA-Interleave, selecting, QBench~\cite{qbench} and BLINK~\cite{blink}.
We systematically evaluated the performance of several current VLMs and our models on these benchmarks. As videos are running in temporal dimension as a natural long-range multimodal tasks, we choose LongVideoBench~\citep{wu2024longvideobenchbenchmarklongcontextinterleaved} and VideoMME~\citep{fu2024videomme}.
\subsection{Data Recipes}
\label{subsec:data-recipes}
\paragraph{Data composition}

Our data is mainly composed of three parts: text long data, MM short data, and video sample data. We aim to explore the impact of these different data types on downstream task performance and, based on this, provide recommended data recipes.
\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{VideoMME} & \textbf{VideoMME} & \textbf{MME} & \textbf{MMBench} \\
 & \textbf{(Long)} & \textbf{(Avg)} & \textbf{(P)} & \textbf{(En)} \\
\midrule
Qwen2-VL-Long & 54.9 & 63.9 & 635.35 & 82.1 \\
\midrule
w/o Short MM Data & 52.1 & 61.2 & 610.47 & 79.8 \\
w/o Video Data & 50.3 & 59.5 & 632.18 & 81.9 \\
w/o Long Text Data & 54.5 & 63.5 & 633.92 & 81.7 \\
\bottomrule
\end{tabular}
}
\caption{Ablation study on different data types for Qwen2-VL-Long}
\label{table:ablation_study}
\end{table}

Table \ref{table:ablation_study} presents an ablation study on the impact of different data types on the performance of Qwen2-VL-Long. The results reveal that each data type contributes uniquely to the model's capabilities. Removing short multimodal (MM) data primarily affects the performance on MME and MMBench tasks, indicating its importance for general visual-language understanding. The absence of video data significantly impacts long video comprehension, as seen in the drop in VideoMME (Long) scores. Interestingly, the removal of long text data has a relatively minor effect across all tasks, suggesting that the model's long-context understanding may be more dependent on multimodal inputs than on pure text. These findings highlight the importance of a diverse training dataset in developing a well-rounded long-context visual language model.



% \begin{tcolorbox}
% \textbf{Findings 1}: Short multimodal instruction data are crucial for maintaining performance on short-form tasks. 
% \end{tcolorbox}

\paragraph{Data ratio}
We further investigated the impact of varying data composition ratios on model performance. Table \ref{table:data_ratio} presents the results of our experiments with different data combinations, where we significantly increased the proportion (60\%) of specific data types: MM instruction data, pure text data, and video data.

\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Data Composition} & \textbf{VideoMME} & \textbf{VideoMME} & \textbf{MME} & \textbf{MMBench} \\
 & \textbf{(Long)} & \textbf{(Avg)} & \textbf{(Acc)} & \textbf{(Dev)} \\
\midrule
Balanced (Qwen2-VL-Long) & 58.5 & 64.8 & 635.35 & 82.1 \\
60\% MM Instruction & 56.7 & 62.1 & 638.12 & 82.3 \\
60\% Pure Text & 56.3 & 61.7 & 620.45 & 80.6 \\
60\% Video & 59.9 & 65.1 & 629.87 & 81.8 \\
\bottomrule
\end{tabular}
}
\caption{Performance of Qwen2-VL-Long with different data composition ratios.}
\label{table:data_ratio}
\end{table}

Our findings indicate that increasing the proportion of MM instruction data does not significantly impact overall performance, with only slight improvements across all tasks. A higher ratio of video data leads to modest gains in video-related tasks (VideoMME) but causes a slight decrease in image-based task performance (MME). Notably, increasing the proportion of pure text data results in a more substantial performance drop across all tasks, suggesting that maintaining a balance of multimodal inputs is crucial for the model's overall capabilities.

% \begin{tcolorbox}
% \textbf{Findings 2}: 
% % In the post-pretraining phase, use a mix of image-text pairs and pure text data. In the post-SFT phase, use collected instruction data.
% \end{tcolorbox}
% \subsection{different training pipeline}
% \paragraph{Freeze VIT or not} weather to freeze it during training
% \begin{table*}[!th]
% \resizebox{\textwidth}{!}{
% % \setlength{\tabcolsep}{3.8pt}
% % \captionsetup{skip=4pt}
% \centering
% \middle

% % \toprule
% % & \multicolumn{4}{c}{Misleading}& \multicolumn{1}{c}{Jailbreak}    & \multicolumn{1}{c}{Harmful Contents} \\
% % \cmidrule(lr){2-5}
% % \cmidrule(lr){6}
% % \cmidrule(lr){7} \\
% % \begin{tabular}{lccccccccccccc}
% % \toprule
% % \multicolumn{1}{l}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Short Visual}} & \multicolumn{1}{c}{\textbf{Long Text}} & \multicolumn{7}{c}{\textbf{Long Visual}}  &\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Avg.}}}\\ 
% % \cmidrule(lr){2-5} \cmidrule(lr){6-6}  \cmidrule(lr){7-12} \cmidrule(lr){13-13} 
% % \multicolumn{1}{l}{} & \multicolumn{2}{c}{MMbench} & \multicolumn{2}{c}{MME} & \multicolumn{1}{c}{\multirow{2}{*}{L-Eval}} & \multicolumn{1}{c}{\multirow{2}{*}{Milebench-T}} & \multicolumn{1}{c}{\multirow{2}{*}{Milebench-S}} & \multicolumn{1}{c}{\multirow{2}{*}{VideoMME-Long}} & \multicolumn{1}{c}{\multirow{2}{*}{VideoMME-S&M}}& \multicolumn{1}{c}{\multirow{2}{*}{MileRuler-QA}}& \multirow{2}{*}{Mileruler-CWE} & \multicolumn{1}{c}{\multirow{2}{*}{Mileruler-VT}}  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
% % \multicolumn{1}{l}{} & \multicolumn{1}{c}{dev} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{acc} & \multicolumn{1}{c}{acc+} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  \\ 
% % % \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{Accuracy} & \multicolumn{3}{c}{Inter annotator consistency} \\ 
% % %  \cmidrule(lr){2-4} \cmidrule(lr){5-7}


% %  % & misleading-text & jailbreak & misleading-img & orderA & orderB & captcha & advise & risk  \\
% % \midrule 

% % \textbf{Qwen-VL-Chat-7B}   \\
% % % \textbf{LLaVA-RLHF-12B} &9.14  &  &  &  &  &  &  &  &  &  &  \\
% % \textbf{Qwen-VL-Long}   \\
% % \textbf{Qwen2-VL-Long}
% % \\
% %  \quad unfreeze VIT   \\
% % \textbf{GPT4V} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} &
% % \textbf{} & \textbf{} &
% % \textbf{} \\
% % \bottomrule
% % % & - & - & - & - & - & - & - & - & - & - \\

% % % & - & - & - & - & - & - & - & - & - & - \\
% % \end{tabular}
% % }
% % \caption{\textbf{VLMs' scores on various short visual tasks, long text tasks and long visual tasks}. The best results are in bold, and the second-best results are underlined. }
% % \label{table:main_table}
% % \end{table*}
% % \mukai{need experiments}

% \begin{tcolorbox}
% \textbf{Findings 3}: .It is better not to freeze vit in most cases
% \end{tcolorbox}
\subsection{Training setting}
\label{subsec:training-setting}
\paragraph{Ablation of Progressive Extension}
We conducted comparative experiments on Qwen-VL to evaluate two methods for extending the model's context length: a single-stage approach and a progressive multi-stage approach. Both methods were controlled for the same number of training steps. The results are summarized in Table \ref{tab:extension_comparison}.

\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{MME\_P} & \textbf{MME\_c} & \textbf{VideoMME} \\
\midrule
Single-stage (128k) & 1462.58 & 350.71 & 48.9 \\
Progressive (8k$\rightarrow$128k) & \textbf{1487.58} & \textbf{360.71} & \textbf{51.2} \\
\bottomrule
\end{tabular}%
}
\caption{Comparison of single-stage and progressive multi-stage extension methods on Qwen-VL.}
\label{tab:extension_comparison}
\end{table}

Our experiments demonstrate that the progressive multi-stage approach consistently outperforms the single-stage method across all evaluated metrics. This suggests that gradually increasing the context length during training allows the model to better adapt to longer sequences, resulting in improved performance on various tasks.

% \begin{tcolorbox}
% \textbf{Findings 4}:In the post-pretraining phase, use a mix of image-text pairs and pure text data. In the post-SFT phase, use collected instruction data.
% \end{tcolorbox}
% \paragraph{Full Finetuning or LoRA}
% test which setting can get the balance between performance and speed.

% \paragraph{Extending LLM base first or not}
% We explored whether extending the length of a VLM requires first extending the length of the LLM base. We tested this by first extending the Qwen base model's length using WikiText, following the same progressive length settings to extend it to 128k. After that, we trained the VLM on the same ExVLM data at a length of 128k.
% \begin{tcolorbox}
% \textbf{Findings 5}: Fixing toplayer of the llm and using sft will drop the performance
% \end{tcolorbox}
\paragraph{Different Position Embedding extending methods}

We conducted a comparative analysis of various methods for extending the context length of visual language models, focusing on their performance on the VideoMME long-range task. Table \ref{tab:position_embedding_comparison} summarizes our findings.

\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \multicolumn{5}{c}{\textbf{VideoMME Long Score (Frames)}} \\
\cmidrule(lr){2-6}
 & 64 & 128 & 256 & 512 & 768 \\
\midrule
Direct extrapolation & 52.5 & 54.3 & 56.2 & 56.4 & 56.5 \\
Origin RoPE & 52.4 & 52.2 & 54.1 & 55.2 & 55.2 \\
PI training & 52.7 & 54.6 & 56.7 & 57.0 & 57.1 \\
M-RoPE NTK & \textbf{53.4} & \textbf{55.9} & \textbf{57.5} & \textbf{58.5} & \textbf{58.5} \\
\bottomrule
\end{tabular}
}
\caption{Comparison of position embedding extension methods on VideoMME long video task on Qwen2-VL.}
\label{tab:position_embedding_comparison}
\end{table}

Our results demonstrate that the M-RoPE interpolation method consistently outperforms other approaches, showing continued improvement as the number of frames increases. This suggests that M-RoPE effectively captures long-range dependencies in video data.

Interestingly, training with original RoPE approach also shows decent performance, likely due to M-RoPE's temporal dimension operating in the high-frequency signal range of RoPE. According to insights from YARN and NTK papers, direct interpolation in this range can affect high-frequency signal expression, potentially leading to performance degradation. However, the temporal nature of video data may mitigate this effect to some extent.

The PI training and direct extrapolation methods show moderate improvements over the baseline, but fall short of M-RoPE's performance. This underscores the importance of carefully considering the unique characteristics of multimodal data when extending position embeddings for visual language models.





\paragraph{Impact of RoPE Base}

We investigated the effect of different RoPE bases on the performance of our extended VLM. Our findings indicate that the optimal performance was achieved by following the recommendations from Su's blog, specifically using a RoPE base of 500,000 for a context length of 128k. Increasing the base beyond this point did not yield significant improvements, while keeping the default base of 10,000 resulted in a notable performance drop. Table \ref{tab:rope_base_comparison} summarizes our results.

\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{RoPE Base} & \textbf{VideoMME Long} & \textbf{VideoMME Avg} & \textbf{MME Sum} & \textbf{MMBench} \\
\midrule
10,000 (default)  & 39.5  & 41.1 & 1848.29 & 60.9 \\
500,000 (optimal)  & \textbf{43.2}  & \textbf{51.2}& \textbf{1862.62} & \textbf{61.5} \\
1,000,000 & 43.1 & 51.1  & 1862.20 & 61.4 \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison of different RoPE bases across various benchmarks.}
\label{tab:rope_base_comparison}
\end{table}

These results underscore the significance of meticulously adjusting the RoPE base when expanding the context window of visual language models. Our findings corroborate the conclusions presented in Su's blog \citep{kexuefm-10122}, which posits that for models with a context length of 128k, an optimal RoPE base of $4.9 \times 10^6$ is recommended. This value closely approximates our selected base of $5 \times 10^5$, which consistently demonstrates superior performance compared to the default configuration across all evaluated metrics.

Interestingly, further increasing the base beyond this point does not yield significant performance improvements. This observation is consistent with the approaches taken by models like LLaMA 2 and Qwen, which have opted for even larger base values. Such choices may provide additional flexibility for future extensions of model context lengths.

The effectiveness of the optimized RoPE base in capturing long-range dependencies in multimodal data underscores the critical role of position embedding strategies in enhancing the performance of extended visual language models.

\subsection{Inference}
\label{subsec:inference}
\paragraph{How to use long context window in VLM}
When encoding videos with a fixed total number of visual tokens, there is a trade-off between the number of frames and the resolution of each frame. According to the Qwen-VL-2 report \citep{wang2024qwen2vlenhancingvisionlanguagemodels}, image task performance often plateaus after reaching a certain resolution, with further increases in visual tokens yielding diminishing returns. We investigated this trade-off by fixing the total visual token usage at approximately 61,440 tokens for video encoding and varying the number of frames while adjusting the resolution accordingly.

Table \ref{tab:frame_resolution_tradeoff} presents the performance of Qwen2-VL-Long on the VideoMME medium and long tasks across different frame counts.

\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Frame Count} & \textbf{Image Token Count} & \textbf{VideoMME Medium} & \textbf{VideoMME Long} \\
\midrule
128 & 480 & 62.5 & 55.6 \\
256 & 240 & 63.9 & 57.3 \\
512 & 120 & 64.6 & 58.2 \\
768 & 80 & \textbf{64.8} & \textbf{58.5} \\
1024 & 60 & 64.7 & \textbf{58.5} \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison of different frame counts and resolutions on VideoMME tasks.}
\label{tab:frame_resolution_tradeoff}
\end{table}

Our findings indicate that for medium-length tasks, performance peaks at 512 frames, with no significant improvements observed beyond this point. However, for long-range tasks, performance continues to improve up to 768 frames, albeit with diminishing returns. This suggests that longer tasks benefit from a higher temporal resolution, even at the cost of reduced spatial resolution per frame.

These results highlight the importance of carefully balancing frame count and resolution when encoding videos for different task lengths. For medium-range tasks, a moderate frame count with higher resolution per frame appears optimal, while long-range tasks benefit from a higher frame count to capture extended temporal dependencies.


\paragraph{Impact of hybrid-inference}
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Frame Count} & \textbf{Image Token Count} & \textbf{VideoMME Medium} & \textbf{VideoMME Long} \\
\midrule
128 & 480 & 62.5 & 55.6 \\
256 & 240 & 63.9 & 57.3 \\
512 & 120 & 64.6 & 58.2 \\
768 & 80 & \textbf{64.8} & \textbf{58.5} \\
1024 & 60 & 64.7 & \textbf{58.5} \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison of different frame counts and resolutions on VideoMME tasks.}
\label{tab:hybrid}
\end{table}

% \begin{tcolorbox}
% \textbf{Findings 6}: Several rope-based extrapolation training methods have little performance difference, and modifying the rope base is a general choice
% \end{tcolorbox}
% \subsection{The effect of ROPE base}
% \mukai{test different rope base }

% 

% \subsection{Long VLM length extraploration}
% text

% \begin{table*}[!th]
% \resizebox{\textwidth}{!}{
% % \setlength{\tabcolsep}{3.8pt}
% % \captionsetup{skip=4pt}
% \centering
% \middle

% % \toprule
% % & \multicolumn{4}{c}{Misleading}& \multicolumn{1}{c}{Jailbreak}    & \multicolumn{1}{c}{Harmful Contents} \\
% % \cmidrule(lr){2-5}
% % \cmidrule(lr){6}
% % \cmidrule(lr){7} \\
% \begin{tabular}{lccccccccccccc}
% \toprule
% \multicolumn{1}{l}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Short Visual}} & \multicolumn{1}{c}{\textbf{Long Text}} & \multicolumn{7}{c}{\textbf{Long Visual}}  &\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Avg.}}}\\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-6}  \cmidrule(lr){7-12} \cmidrule(lr){13-13} 
% \multicolumn{1}{l}{} & \multicolumn{2}{c}{MMbench} & \multicolumn{2}{c}{MME} & \multicolumn{1}{c}{\multirow{2}{*}{L-Eval}} & \multicolumn{1}{c}{\multirow{2}{*}{Milebench-T}} & \multicolumn{1}{c}{\multirow{2}{*}{Milebench-S}} & \multicolumn{1}{c}{\multirow{2}{*}{VideoMME-Long}} & \multicolumn{1}{c}{\multirow{2}{*}{VideoMME-S&M}}& \multicolumn{1}{c}{\multirow{2}{*}{MileRuler-QA}}& \multirow{2}{*}{Mileruler-CWE} & \multicolumn{1}{c}{\multirow{2}{*}{Mileruler-VT}}  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
% \multicolumn{1}{l}{} & \multicolumn{1}{c}{Text} & \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{\ding{51}- \ding{55}} & \multicolumn{1}{c}{\ding{55}-\ding{51}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  \\ 
% % \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{Accuracy} & \multicolumn{3}{c}{Inter annotator consistency} \\ 
% %  \cmidrule(lr){2-4} \cmidrule(lr){5-7}

%  % & misleading-text & jailbreak & misleading-img & orderA & orderB & captcha & advise & risk  \\
% \midrule 

% \textbf{Qwen-VL-Chat-7B} \\
% \textbf{Qwen-VL-Long}   \\
% \quad \textbf{w/o text long data}\\

% \quad \textbf{w/o MM short data} \\

% \quad \textbf{w/o MM interleave data} \\

% \quad \textbf{w/o video data} &  \\

% % \textbf{LLaVA-RLHF-12B} &9.14  &  &  &  &  &  &  &  &  &  &  \\

% % &{\underline{8.73}}	&{\underline{5.51}}	&{\underline{6.42}}	 &{\underline{6.81}}	&{\underline{5.95}}	&6.72	&7.42	&8.28	&5.32	&{\underline{7.32}}	&{\underline{6.95}}		&7.27	&{\underline{6.89}}

% % & - & - & - & - & - & - & - & - & - & - \\

% % & - & - & - & - & - & - & - & - & - & - \\
% \end{tabular}
% }
% \caption{\textbf{VLMs' scores on various short visual tasks, long text tasks and long visual tasks}. The best results are in bold, and the second-best results are underlined. }
% \label{table:main_table}
% \end{table*}

% Using RoPE positional encoding, long VLMs have a certain degree of extrapolation capability. We tested the results on MileBench at different lengths to determine the range of the VLM’s length extrapolation ability.

% We investigated the performance of using LoRA and full fine-tuning to train long VLMs. To save memory, we fixed the lower layers of the LLM and only trained the higher layers.

% \mukai{add newer exp results here}



% \begin{tcolorbox}
% \textbf{Findings 6}:The performance of the vlm using the rope for extrapolation degrades slowly, with a significant drop in performance after about twice the length.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/data_table.tex <==
\begin{table*}[]
\begin{tabular}{llllllllllllll}
\tiny
 & \multicolumn{2}{l}{Short eval} & \multicolumn{8}{l}{Long eval} &  &  &  \\
 & choice & Single hop trace & Single hop trace & \multicolumn{4}{l}{choice} & Aggregation & Multi-hop Tracing & Long QA &  &  &  \\
 & MMBENCH-dev & VLMhaystack & VLMhaystack-64k-milebench & milebench-t & milebench-s & Video mme long-first w/o sub & Video mme long-first w sub & milebench-ruler-CWE & milebench-ruler-VT &  &  &  &  \\
qwen-vl &  &  &  &  &  &  &  &  &  &  &  &  &  \\
qwen-vl-ring-128k &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  & 
\end{tabular}
\end{table*}
